Leveraging Large Language Models for Automated Dialogue Analysis

Developing high-performing dialogue systems benefits from the automatic identification of undesirable behaviors in system responses. However, detecting such behaviors remains challenging, as it draws on a breadth of general knowledge and understanding of conversational practices. Although recent research has focused on building specialized classifiers for detecting specific dialogue behaviors, the behavior coverage is still incomplete and there is a lack of testing on real-world human-bot interactions. This paper investigates the ability of a state-of-the-art large language model (LLM), ChatGPT-3.5, to perform dialogue behavior detection for nine categories in real human-bot dialogues. We aim to assess whether ChatGPT can match specialized models and approximate human performance, thereby reducing the cost of behavior detection tasks. Our findings reveal that neither specialized models nor ChatGPT have yet achieved satisfactory results for this task, falling short of human performance. Nevertheless, ChatGPT shows promising potential and often outperforms specialized detection models. We conclude with an in-depth examination of the prevalent shortcomings of ChatGPT, offering guidance for future research to enhance LLM capabilities.

==> latex/costs.tex <==

\section{Cost Comparison}

Table \ref{tab:cost_comparison} shows the average cost to collect behavior labels for a single conversation using ChatGPT or human evaluators. ChatGPT boasts extreme cost-efficiency relative to humans, reducing the cost by at least an order of magnitude for each behavior. Even with the proposed mitigation strategies in \S\ref{sec:recommendations} leading to an increase in overall prompt length, such cost savings would still persist. This potential for substanstial price reductions makes future work on improving ChatGPT performance even more desirable, as even specialized classifiers rely on human annotations for training creation which ends up being quite costly.

==> latex/old/error_analysis.tex <==
    %  &  &  &  &  &  &  &  &  &  &  &  \\
    % World knowledge detection & 9 & - & - & - & - & - & - & - & - & 9 & 0.03 \\
    %  &  &  &  &  &  &  &  &  &  &  &  \\
    % Emotional salience & - & - & - & - & - & - & 3 & - & - & 3 & 0.01 \\
    % Emotional tone & - & - & - & - & - & - & 3 & - & - & 3 & 0.01 \\
    %  &  &  &  &  &  &  &  &  &  &  &  \\
    % Validative Followup & - & - & - & - & - & - & - & - & 14 & 14 & 0.05 \\
    % Emotion Mimicry & - & - & - & - & - & - & - & - & 4 & 4 & 0.01

==> latex/old/error_analysis_2.tex <==

\section{GPT Error Analysis}
\label{sec:gpt_error_analysis}

We conduct an error analysis of the dialogue behavior predictions made by GPT in order to better understand its current limitations. For each dialogue behavior, we take 40 instances in which GPT disagreed with the human label and examine the reasoning outputted by the GPT model before it made its final decision. We construct a set of dialogue characteristics and GPT predispositions into which each mistake can be categorized, which are shown in Table \ref{tab:error_analysis}.

\begin{table*}[h]
    \centering\small
    \begin{tabular}{l||c|c|c|c|c|c|c|c|c||c|c}
    & \textbf{!Fac} & \textbf{Red} & \textbf{!Com} & \textbf{!Rel} & \textbf{!Par} & \textbf{!Sel} & \textbf{!Emp} & \textbf{Ign} & \textbf{Emp} & $\bm{\Sigma}$ & \bf \%\\
    \hline \hline 
    Inexperience          & 18 & -  & 14 & 10 & 3  & 7  & -  & 9  & 2  & 63 & 0.18 \\
    History Forgetfulness & -  & 21 & 9  & -  & 19 & 1  & -  & 1  & -  & 51 & 0.14 \\
    Disassociated Context & 1  & -  & -  & 7  & 6  & -  & 2  & 14 & 1  & 31 & 0.09 \\
    Selective Attention   & -  & 2  & 2  & 3  & 1  & -  & 8  & 7  & 10 & 33 & 0.09 \\
    Definition Mismatch   & 1  & 2  & 4  & 1  & 2  & 8  & 1  & 2  & -  & 21 & 0.06 \\
    Semantic Relatedness  & -  & 9  & -  & 2  & -  & 1  & 7  & -  & -  & 19 & 0.05 \\
    Conversation Norms    & -  & 1  & -  & 13 & 2  & -  & -  & -  & 1  & 17 & 0.05 \\
    Mutual Exclusion      & -  & -  & 3  & -  & 2  & 8  & -  & -  & -  & 13 & 0.04 \\
    Role Confusion        & -  & 2  & 1  & -  & 2  & 7  & -  & -  & 1  & 13 & 0.04 \\
    Exhaustive            & -  & -  & -  & -  & -  & -  & 3  & 3  & 4  & 10 & 0.03 \\
    Misidentification     & -  & 2  & 1  & 1  & 1  & 2  & 1  & 2  & 2  & 12 & 0.03 \\
    Temporal Framing      & -  & -  & 5  & -  & 2  & -  & -  & -  & -  & 7  & 0.02 \\
    Reasoning Mismatch    & -  & -  & -  & 3  & -  & 1  & 2  & 1  & -  & 7  & 0.02 \\
    Claim Detection       & 3  & -  & -  & -  & -  & 1  & -  & -  & -  & 4  & 0.01 \\
    Over-analysis         & 1  & -  & -  & -  & -  & 3  & -  & -  & -  & 4  & 0.01 \\
    Confused Target       & -  & 1  & -  & -  & -  & -  & -  & 1  & 1  & 3  & 0.01 \\
    Bot Identity          & -  & -  & 1  & -  & -  & 1  & -  & -  & -  & 2  & 0.01 \\
\end{tabular}
    \caption{Results of the error analysis on GPT's reasoning for dialogue behavior detection.}
    \label{tab:error_analysis}
\end{table*}

\begin{quote}
\small
(S1) no i dont have any hobbies

(S2) Oh, okay. I heard you say hobbies. That is a great thing to do to keep yourself busy, especially in these times! What do you like so much about this hobby?

(S1) i dont have any. do you?

(S2) That makes sense. For me personally, I've been taking the time to read a little bit every day. It was slow going at first, but now I really enjoy it.

(R) Speaker 2 asks Speaker 1 about their hobbies and then assumes that they have a hobby they enjoy. However, Speaker 1 responds by saying they don't have any hobbies. Speaker 2 then asks what Speaker 1 likes about their hobby, which is a repetitive question since Speaker 1 already stated they don't have any hobbies. Therefore, Speaker 2 has contradicted what Speaker 1 has already shared.
\end{quote}

The predominant cause of GPT's errors is its inability to attend to the most relevant segments of the dialogue and utterance in question. 33\% of the issues that GPT made can be traced back to it seemingly forgetting some information shared previously in the history (\textbf{History Forgetfulness}), incorrectly remembering the order of the conversation (\textbf{Disassociated Context}), completely overlooking sentences in a compound response (\textbf{Selective Attention}), or confusing which utterance it is labelling in the current moment (\textbf{Confused Target}).

\begin{figure}[H]
    \centering
    \includegraphics[width=\columnwidth]{latex/img/confused_target.pdf}
    \caption{Caption}
    \label{fig:my_label}
\end{figure}

GPT also demonstrates a large degree of (\textbf{Inexperience}) (18\% of mistakes), as its reasoning often reveals a lack of wisdom about human experiences, which can lead to having too high of standards for certain labels or misunderstanding nuances of situations. For \texttt{!Fac}, this inexperience manifests as a lack of accurate knowledge about the world, as GPT often misses when an incorrect statement is made. For other labels, it manifests as a lack of general knowledge, leading to the drawing of faulty conclusions. For instance, in one case, GPT explained its decision to not label a particular response as \texttt{!Com} because "It is a common response to wish someone a good trip even if they have not planned one yet", which is obviously incompatible with human understanding. 

Another significant cause is GPT's lack of conceptual understanding. 16\% of the issues that GPT made can be traced back to it misunderstanding the degree of similarity between two ideas (\textbf{Semantic Relatedness}), misidentifying when two events or concepts can or cannot co-occur together (\textbf{Mutual Exclusion}), confusing the specified timeline of a particular situtation, such as by assuming characteristics of a concluded event are occurring currently (\textbf{Temporal Framing}), or misunderstanding what constitutes an acceptable coherence in a particular progression of dialogue (\textbf{Conversation Norms}). 

9\% of GPT's mistakes can be explained by it misinterpreting the dialogue context, either by misunderstanding the intent of what has been shared (\textbf{Misidentification}), reading too much into what has been said previously such that unsupported conclusions are made (\textbf{Over-analysis}), incorrectly identifying that a claim/statement is being made (\textbf{Claim Detection}), or confusing the speaker of previous utterances (\textbf{Role Confusion}).

% misidentification --> good example is in irrelevant

In 10\% of cases, there was a mismatch between GPT's definition of the dialogue behavior and its true definition, where GPT either assumed all examples provided in the definition in the prompt must be met for the behavior to occur (\textbf{Exhaustive}), considered indicators of Speaker 2 being a bot as applicable behavior for certain behaviors like commonsense contradictions (\textbf{Bot Identity}), or otherwise expanded beyond the provided definition of the behavior such as by considering meta-level characteristics of the dialogue rather than the actual response semantics (\textbf{Definition Mismatch}).

Finally, in a minority of cases (2\%), GPT exhibited inconsistent internal reasoning, where its explanation was at-odds with the final decision it produced  (\textbf{Reasoning Mismatch}).

Certain GPT mistakes were isolated to one dialogue behavior, rather than occurring across several. \texttt{!Fac} was often limited by GPT's inability to detect when a claim about world knowledge is being given, often labelling personal knowledge as incorrect facts ($n=16$). \texttt{Emp} was inhibited by GPT's preconception that a follow-up question or response was \textit{not} enough to warrant an empathetic label, whereas human judges believed the opposite ($n=14$). Finally, GPT displayed a lack of emotional understanding ($n=16$) - including not identifying when an experience was emotionally salient, not recognizing what exact emotions an experience provoked in the speaker, or overlooking when the sharing of personal experiences or asking questions was distastefully done - that prevented it from identifying cases of \texttt{!Emp}.  

\begin{figure*}[t]
\centering
\begin{subfigure}{0.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{latex/img/confused_target.pdf}
\end{subfigure}%
\begin{subfigure}{0.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{latex/img/disassociated_context_3.pdf}
\end{subfigure}
\caption{}
\label{fig:error_analysis_examples}
\end{figure*}

\begin{table*}[h]
    \centering\small
    \begin{tabular}{c|p{6cm}|p{7cm}}
     & Dialogue & Reasoning \\
    \hline
    !Exp & (1) I don't have a trip planned, but maybe I'll go somewhere soon \newline (2) I'm sure you will! You'll love it! Have a wonderful trip! I'll see you soon! & The response does not contradict commonsense as it is a polite and friendly response to the previous statement. It does not make any unfounded assumptions, is not illogical or self-contradictory, and does not ask a question where the answer is already obvious. It is a common response to wish someone a good trip even if they have not planned one yet. \newline\newline \texttt{!Com}: 1 [Inexperienced] \\
    \hline
    !His & (1) I do! I have a younger brother. What about you? \newline (2) You have a brother? Cool! Do you guys get along? \newline (1) We used to fight a lot as kids, but we get along well now. \newline (2) That's awesome. Personally, I always wanted an older sister so I could have someone to look up to. Are you older than your brother? & The response asks a new question that has not been answered yet, which is whether Speaker 1 is older than their brother. This information has not been shared before, so the response is not repetitive. \newline\newline \texttt{Red} [1] \\
    \hline
    !Tar & (1) no i dont have any hobbies \newline (2) Oh, okay. I heard you say hobbies. That is a great thing to do to keep yourself busy, especially in these times! What do you like so much about this hobby? \newline (1) i dont have any. do you? \newline (2) That makes sense. For me personally, I've been taking the time to read a little bit every day. It was slow going at first, but now I really enjoy it. & Speaker 2 asks Speaker 1 about their hobbies and then assumes that they have a hobby they enjoy. However, Speaker 1 responds by saying they don't have any hobbies. Speaker 2 then asks what Speaker 1 likes about their hobby, which is a repetitive question since Speaker 1 already stated they don't have any hobbies. Therefore, Speaker 2 has contradicted what Speaker 1 has already shared. \newline\newline \texttt{!Par} [0] \\
    \hline
    Dis & (2) I'm sure you'll feel great after your workout! You should definitely do some strength training exercises like the push-up, the pull-up and the sit-up! They're some of the most common bodyweight exercises! \newline (1) Yes! What's your favourite color? \newline (2) I'm not sure about you, but my favorite color is blue! I like it because it reminds me of the color of the sea! & Speaker 1 asked about dinner, and Speaker 2 responded by saying they haven't had dinner yet and then shifted the topic to working out. Speaker 2 then asked about Speaker 1's favorite exercises at the gym. Speaker 1 did not mention anything about favorite colors, so Speaker 2's response is completely off-topic and does not address the previous turn from Speaker 1. \newline\newline \texttt{Ign} [0] \\
    \hline
    !Att & (2) I love pop! What is your favorite r\&b artist? Do you like nicki minaj? \newline (1) I do like Nicki! \newline (2) I like her too, she's so talented. Do either of your parents work? My mom is a teacher. & Speaker 2 does not demonstrate any understanding of Speaker 1's emotions or react with an appropriate sentiment or emotion to Speaker 1's shared experience. Instead, Speaker 2 changes the subject to ask about Speaker 1's parents. This response is not empathetic. \newline\newline \texttt{Emp} [1] \\
    \hline
    Sem & (2) You have a brother? Cool! Do you guys get along? \newline (1) We get along pretty well but fight sometimes \newline (2) That kind of sounds like my friend grace, she loves her younger brother but they fight all the time. What does your brother do that bothers you? & Speaker 2's response shows an attempt to relate to Speaker 1's experience by bringing up their friend Grace who also fights with her younger brother. However, Speaker 2 does not directly acknowledge or address Speaker 1's feelings about their own relationship with their brother. Therefore, Speaker 1 may feel like their feelings are not being fully understood by Speaker 2. \newline\newline \texttt{!Emp} [0] \\
    \hline
    !Def & (1) Yes, I'm in a few clubs. What about you? \newline (2) I'm not in any clubs right now. I haven't found one that really suits me. \newline (1) I'm sure you'll find one soon enough. \newline (2) Uh-huh. Wait, did you say you were in any school clubs? & Speaker 2's question, "Wait, did you say you were in any school clubs?" is a self-contradiction because in line 30, Speaker 1 explicitly stated that they are in a few school clubs. Speaker 2's question contradicts this information and shows a lack of attention or memory. \newline\newline \texttt{!Sel} [0] \\
    \hline
    Nor & (1) Hi! \newline (2) hi! I am happy to be talking to you. I hope you don't mind me asking, but are you dating anyone right now? & The response from Speaker 2 is completely irrelevant to what Speaker 1 said. Speaker 1 simply greeted Speaker 2 and did not provide any information that would lead to a discussion about dating. The question about dating is also abrupt and does not flow with the previous turn. \newline\newline \texttt{!Rel} [0] \\
    \hline
    
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table*}



==> latex/old/related_work.tex <==
\section{Related Work}

\subsection{Speaker Contradiction Detection}
\label{sec:rw_speaker_contradiction}

There has been much interest in enabling dialogue systems to maintain a consistent persona through their responses \cite{personachat, others, shuster:22, kim:20}. Beyond persona-grounded dialogue, some response generation works explicitly model important information shared in the dialogue context as the dialogue progresses and integrate such memory as additional context for response generation in order to reduce contradictions \cite{xu_long:22, xu_beyond:22}.

In terms of specific approaches to response contradiction detection, many of these works also focus on detecting contradictions to a given persona \cite{shuster:22, welleck:19, song:20}. \citet{shuster:22} propose a role-playing-accuracy classifier which identify whether a dialogue response belongs to the correct persona out of a set of personas. \citet{welleck:19} construct Dialogue Natural Language Inference (DNLI) dataset automatically from PersonaChat by aligning dialogue utterances to their persona sentences based on human-annotated triple-representations of persona-information into 3 categories: \textit{entailment}, \textit{contradiction}, or \textit{neutral} relationships. \citet{song:20} utilize an NLI model trained on DNLI to identify the words in a dialogue response that are the source of the contradiction.

Beyond persona-grounded dialogues, NLI-based models are still commonly used to detect history contradictions \cite{li:21, nie:21} with \citet{nie:21} developing a RoBERTa classification model\footnote{\href{https://huggingface.co/ynie/roberta-large_conv_contradiction_detector_v0}{https://huggingface.co/ynie/roberta-large\_conv\_contradiction\_detector\_v0}} trained on DECODE - a contradiction dataset for dialogue where human annotators wrote contradictory and non-contradictory dialogue responses with respect to the current speaker's previous utterances in the dialogue. On the other hand, \citet{shi:21} utilize a key-value based inconsistency detector, where key-value profiles are built and compared for each speaker as the dialogue progresses using domain-specific dialogue-act classifiers. Their profiles are specifically curated for their dialogue task (monetary donation persuasion) and are quite small, with only 5 attributes being tracked. Furthermore, \citet{zheng:22} decompose contradiction detection into a more fine-grained detail with 3 categories - intra-sentence contradiction, role confusion, and history contradiction - and create CDConv, a dataset of annotated Chinese dialogues.

Notably, these existing approaches to contradiction detection fail to address the task of partner contradictions, instead focusing on whether the dialogue responses contradict the speaker's persona or previous utterances (other than \cite{shi:21} which is too restricted to be generally applicable to any dialogue).

\subsection{Commonsense Contradiction Detection}
\label{sec:rw_commonsense_contradiction}

Entailment - commonsense contradictions



\subsection{Claim Verification}
\label{sec:rw_claim_verification}

There is much interest in claim verification for NLG tasks \cite{fill}. We focus specifically on the works pertaining to claim verification in dialogue. Although some works focus on claim verification for (question, response) pairs \cite{wang:22}, we focus on works that incorporate more diversity in dialogue interaction types.

Most works on detecting incorrect facts in dialogue focus exclusively on dialogue responses that incorporate knowledge and assume that the grounding knowledge text is given. \citet{gupta:22} propose two additional precursor tasks to claim verification that are necessary in practice - verifiable claim detection and evidence selection - and presents results of various methodologies on these tasks, as well as on claim verification. In addition, they present their DialFact dataset, which is intended to only be used for evaluation purposes. Their proposed claim verification model (Bert finetuned on their synthetically constructed dataset Aug-Wow) outperforms baseline models on claim verification on DialFact. They do not compare to other dialogue claim verification models, though, instead comparing to dialogue consistency models and non-dialogue claim verification.

\citet{dziri_begin:22} propose BEGIN, a dataset of dialogue responses generated from knowledge-grounded dialogue systems and annotated for their faithfulness to grounding knowledge text, which is intended to be used only for evaluation purposes. They evaluate various claim verification approaches, including lexical overlap, embedding similarity, question-answering, and trained classifiers. They construct an adversarial training dataset (BEGIN-Adversarial) using the original human utterances from WoW and various perturbing strategies. They find that classifier-based approaches perform the best on BEGIN, especially when trained on BEGIN-Adversarial, although still far from human performance. They outperform against models trained on AugWow.

\citet{dziri_faithdial:22} propose FaithDial, a dataset of WoW dialogues where the unfaithful dialogue responses were edited by humans to be faithful to their grounding knowledge texts, and derive a claim verification dataset from it - Faith-Critic - using the original responses that were labelled as unfaithful as negative examples and those labelled as faithful as positive examples, along with the human-edited versions -- 34K total. They finetune a RoBERTa model on claim verification using Faith-Critic and observe that it outperforms baseline models, even when evaluated on other claim verification datasets like BEGIN. They do no compare to other dialogue claim verification models, though, instead comparing to dialogue consistency models.


\subsection{Empathy}
\label{sec:rw_empathy}

Empathetic response generation is a popular task for conversational AI and when evaluating the empathy (or lack thereof) produced by such works, human judges are commonly used \cite{zhong:20,sabour:22,qian:23}. In much less quantity, there has been some work on automatic identification of empathetic responses. \citet{welivita:20} develop a taxonomy for response intents specific to empathetic responses and use n-gram string matching to automatically label all utterances in EmpatheticDialogues based on 500 manually labelled dialogues.  \citet{svikhnushina:22} develop a taxonomy of questions used in empathetic responses and then crowdsource annotations for 6K questions taken from EmpatheticDialogues, before augmenting the labelled data by automatically labelling the remainder of the EmpatheticDialogues dataset using k-Nearest-Neighbors. Although such work is useful for analyzing \textit{empathetic} responses, it is lacking annotations of \textit{unempathetic} responses that are crucial for being able to distinguish between the two. 

To the best of our knowledge, \citet{sharma:20} is the only existing dataset that specifically seeks to identify whether a response is empathetic or not. \citet{sharma:20} collect EPITOME - a dataset of 10K (post, response) pairs from TalkLife and Reddit that are annotated with the strength of their expression - no expression, weak expression, and strong expression - of 3 empathetic communication mechanisms - reactions, interpretations, and explorations. Only the Reddit portion (3K) is publicly available. They train one multi-task RoBERTa-based bi-encoder model for expression classification and rational extraction for each communication mechanism, and show that it outperforms baseline models on these tasks. Some recent works on empathetic response generation have utilized these trained classifiers in their approaches \cite{zheng:21, majumder:22} or as automatic evaluation methods \cite{kim:21, lee:22}. 

\subsection{Coherence}
\label{sec:rw_coherence}

The Dialogue Breakdown Detection Challenge (DBDC) is a chat-oriented evaluation workshop focusing on the detection of chatbot utterances that impede the continuation of the conversation due to their inappropriateness in the context \cite{higashinaka:19}. Several iterations of DBDC have been conducted, with the most recent being DBDC5 in 2020. On DBDC5, \citet{lin:22} achieve the highest reported performance to date, outperforming the detection model that placed first during the timeframe of the actual challenge \cite{ng:20}. Although the annotated breakdowns are not necessarily exclusively due to coherence issues, observations of the dataset suggest that they are a dominant cause.

Relative to other dialogue behaviors, there is little work on detecting specific incoherent behaviors: ignoring the previous turn, being irrelevant to the context, or being redundant. In the rest of this section, we highlight the relevant works for such detection tasks.

\paragraph{Ignore and Irrelevant}

\citet{xu:21} incorporate an incoherence detection task as a self-supervised training objective for improving dialogue model response generation. Given a corpus of dialogues, utterances are randomly replaced with other utterances in the corpus. The incoherence detection model is then tasked with correctly selecting which utterance was replaced within a dialogue.

\paragraph{Redundant}

Several approaches have been proposed to reduce token/n-gram repetition in dialogue response generation \cite{li:20, xi:21} and to reduce repetitive incorporation of the same knowledge text in multi-turn dialogues \cite{sun:20}; however, these tasks target end-to-end response generation and do not treat redundancy detection itself as a task. 

Towards redundancy detection, \citet{shi:21} use the Jaccard similarity coefficient between a response and the turns in the dialogue history as a measurement of a response's redundancy. They report that they experimented with sentence embedding approaches too, but found that they were less effective for their dialogue task (i.e. monetary donation persuasion). However, there has been much work on paraphrase detection and semantic similarity using embeddings that have been successful \cite{fill}.

% \cite{sun:20} address the idea of repetition of external knowledge in dialogue using a gating mechanism to control the incorporation of independent knowledge texts on a particular turn. 

% \citet{li:20} utilize unlikelihood training to reduce contextual and within-response repetitions of n-grams by punishing the production of tokens within these n-grams when calculating the loss during training. Rather than punishing repetition uniformly, \cite{xi:21} develop a response generation model that learns to control when repetition is appropriate or inappropriate given a particular dialogue context.

==> latex/old/results_othermetrics.tex <==

\begin{table*}[h!]
    \centering
    \begin{tabular}{l|l|r|l|l}
    \bf Error & \bf Model & \multicolumn{1}{|c|}{$\bm{\alpha}$} & $\bm{H_{agreed}}$ & $\bm{H_{atodds}}$ \\ \hline \hline
    Self Contra. & GPT & 0.11 & 0.08 / 0.40 / 0.14 & 1.0 / 0.33 / 0.49 \\
    Self Contra. & DECODE & 0.24 & 0.17 / 0.67 / 0.27 & 1.0 / 0.34 / 0.50 \\
    \hline
    Partner Contra. & GPT & 0.13 & 0.21 / 0.18 / 0.19 & 1.0 / 0.11 / 0.20 \\
    % Partner Contra. & DECODE$_{p}$ & &  &  \\
    \hline
    Commonsense & GPT & 0.22 & 0.41 / 0.35 / 0.38 & 1.0 / 0.22 / 0.36 \\
    \hline
    Incorrect Fact & GPT & 0.36 & 0.35 / 0.52 / 0.42 & 1.0 / 0.20 / 0.47  \\
    Incorrect Fact & Faith-Critic & &  &   \\
    \hline
    Empathetic & GPT & -0.05 & 0.51 / 0.12 / 0.20 & 1.0 / 0.12 / 0.21   \\
    Empathetic & EPITOME & -0.14 & 0.36 / 0.86 / 0.51 & 1.0 / 0.86 / 0.92   \\
    \hline
    Lack of Empathy & GPT & 0.09 & 0.16 / 0.44 / 0.23 & 1.0 / 0.28 / 0.44  \\
    Lack of Empathy & EPITOME & -0.03 & 0.08 / 0.18 / 0.11  & 1.0 / 0.13 / 0.22  \\
    \hline
    Redundant & GPT & 0.27 & 0.27 / 0.45 / 0.34 & 1.0 / 0.56 / 0.72 \\
    % Redundant & Embedding+QA & &  &  \\
    \hline
    Ignore & GPT & -0.02 & 0.51 / 0.12 / 0.20 & 1.0 / 0.12 / 0.21  \\
    Ignore & S2T2 & 0.11 & 0.14 / 0.41 / 0.20 & 1.0 / 0.37 / 0.54  \\
    \hline
    Irrelevant & GPT & 0.21 & 0.24 / 0.69 / 0.35 & 1.0 / 0.55 / 0.71 \\
    Irrelevant & S2T2 & 0.11 & 0.17 / 0.36 / 0.24 & 1.0 / 0.30 / 0.47  \\
    \end{tabular}
    \caption{Error detection results on the ABC-Eval dataset. $\bm{\alpha}$: average Krippendorf's alpha with the human annotators. $\bm{H_{agreed}}$: precision/recall/f1-score on the positive labels for which the human annotators agreed. $\bm{H_{atodds}}$: precision/recall/f1-score on the instances for which the human annotators disagreed, if we take them as positive instances.}
    \label{tab:results}
\end{table*}

==> latex/old/results_table.tex <==
\begin{table*}[h!]
    \centering\small
    \renewcommand{\arraystretch}{1.05}
    \begin{tabular}{l|l|r|l|l|l|l|l}
    \bf Error & \bf Model & \multicolumn{1}{|c|}{$\bm{\alpha}$} & \multicolumn{1}{|c|}{\textbf{P$_+$ / R$_+$ / F1$_+$}} & \multicolumn{1}{|c|}{\textbf{P / R / F1}} & \bf Acc & \bf \#$\bm{_p}$ & \bf \#$\bm{_t}$ \\ \hline \hline
    \multirow{3}{*}{\tt !Fac} & GPT & 0.36 & 0.38 / 0.45 / 0.41 & 0.67 / 0.69 / 0.68 & 0.90 & 146 & \multirow{3}{*}{122}\\
    & Faith-Critic & 0.06 & 0.12 / 0.22 / 0.16 & 0.53 / 0.55 / 0.53 & 0.82 & 223 & \\
    & Human & 0.65 & 0.68 / 0.68 / 0.68 & 0.83 / 0.83 / 0.83 & 0.95 & & \\
    \hline
    \multirow{2}{*}{\tt Red} & GPT & 0.27 & 0.31 / 0.35 / 0.33 & 0.63 / 0.64 / 0.63 & 0.89 & 148 & \multirow{2}{*}{129}\\
    & Human & 0.55 & 0.59 / 0.59 / 0.59 & 0.78 / 0.78 / 0.78 & 0.93 & & \\
    \hline
    \multirow{2}{*}{\tt !Com} & GPT & 0.22 & 0.44 / 0.29 / 0.35 & 0.64 / 0.60 / 0.61 & 0.78 & 219 & \multirow{2}{*}{333}\\
    & Human & 0.44 & 0.56 / 0.56 / 0.56 & 0.72 / 0.72 / 0.72 & 0.82 && \\
    \hline
    \multirow{3}{*}{\tt !Rel} & GPT & 0.21 & 0.30 / 0.63 / 0.41 & 0.61 / 0.67 / 0.61 & 0.71 & 543 & \multirow{3}{*}{261}\\
     & S2T2 & 0.11 & 0.24 / 0.33 / 0.28 & 0.55 / 0.57 / 0.55 & 0.72 & 365 & \\
     & Human & 0.46 & 0.54 / 0.54 / 0.54 & 0.73 / 0.73 / 0.73 & 0.85 & \\
    \hline
    \multirow{2}{*}{\tt !Par} & GPT & 0.13 & 0.27 / 0.14 / 0.19 & 0.59 / 0.55 / 0.56 & 0.89 & 79 & \multirow{2}{*}{151}\\
     & Human & 0.45 & 0.49 / 0.49 / 0.49 & 0.72 / 0.72 / 0.72 & 0.91 & & \\
    \hline
    \multirow{3}{*}{\tt !Sel} & GPT & 0.11 & 0.15 / 0.36 / 0.21 & 0.55 / 0.61 / 0.56 & 0.83 & 250 & \multirow{3}{*}{101}\\
     & DECODE & 0.24 & 0.23 / 0.49 / 0.31 & 0.60 / 0.69 / 0.62 & 0.87 & 215 & \\
    & Human & 0.41 & 0.45 / 0.45 / 0.44 & 0.71 / 0.71 / 0.70 & 0.93 & \\
    \hline
    \multirow{3}{*}{\tt !Emp} & GPT & 0.09 & 0.21 / 0.36 / 0.27 & 0.55 / 0.57 / 0.55 & 0.72 & 396 & \multirow{3}{*}{231}\\
    & EPITOME & -0.03 & 0.12 / 0.15 / 0.13 & 0.49 / 0.48 / 0.48 & 0.72 & 291 & \\
    & Human & 0.44 & 0.52 / 0.52 / 0.52 & 0.72 / 0.72 / 0.72 & 0.86 & \\
    \hline
    \multirow{3}{*}{\tt Ign} & GPT & -0.02 & 0.16 / 0.63 / 0.25 & 0.54 / 0.62 / 0.49 & 0.60 & 696 & \multirow{3}{*}{170}\\
     & S2T2 & 0.11 & 0.18 / 0.40 / 0.25 & 0.55 / 0.60 / 0.55 & 0.75 & 365 & \\
     & Human & 0.57 & 0.62 / 0.62 / 0.62 & 0.79 / 0.79 / 0.79 & 0.92 & \\
    \hline
    \multirow{3}{*}{\tt Emp} & GPT & -0.05 & 0.51 / 0.12 / 0.19 & 0.57 / 0.52 / 0.47 & 0.62 & 146 & \multirow{3}{*}{618} \\
     & EPITOME & -0.14 & 0.40 / 0.86 / 0.54 & 0.55 / 0.53 / 0.43 & 0.45 & 1343 &  \\
     & Human & 0.51 & 0.70 / 0.70 / 0.70 & 0.76 / 0.76 / 0.76 & 0.77 & \\
    \end{tabular}
    \caption{Error detection results on the ABC-Eval dataset. $\bm{\alpha}$: average Krippendorf's alpha against human annotators. \textbf{P$_+$ / R$_+$ / F1$_+$}: average precision/recall/f1 on human-annotated positive labels. \textbf{P / R / F1}: average macro-precision/recall/f1-score on human-annotated labels. \textbf{Acc}: average accuracy on the human-annotated labels. \textbf{\#$_p$}: number of positive labels predicted by model. \textbf{\#$_t$}: average number of positive labels annotated by human. }
    \label{tab:results}
\end{table*}

==> latex/old/results_table_2.tex <==
\begin{table}[ht]
    \centering\small
    % \renewcommand{\arraystretch}{1.05}
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{r||l|r|l|l|l|l}
    & \bf Model & \multicolumn{1}{|c|}{$\bm{\alpha}$} & \multicolumn{1}{|c|}{\textbf{P$_+$ / R$_+$ / F1$_+$}} & \multicolumn{1}{|c|}{\textbf{F1}} & \bf Acc & \bf \#$\bm{_p}$ \\
    \hline \hline % &&&&&& \\
    \multirow{3}{*}{\tt !Fac} & FC & 0.06 & 0.12 / 0.22 / 0.16 & 0.53 & 0.82 & 223   \\
    & GPT & 0.36 & 0.38 / 0.45 / 0.41 & 0.68 & 0.90 & 146 \\
    & HUM & 0.65 & 0.68 / 0.68 / 0.68 & 0.83 & 0.95 & 122 \\
    \hline %&&&&&& \\ 
    \multirow{2}{*}{\tt Red} & GPT & 0.27 & 0.31 / 0.35 / 0.33 & 0.63 & 0.89 & 148 \\
    & HUM & 0.55 & 0.59 / 0.59 / 0.59 & 0.78 & 0.93 & 129 \\
    \hline %&&&&&& \\
    \multirow{2}{*}{\tt !Com} & GPT & 0.22 & 0.44 / 0.29 / 0.35 & 0.61 & 0.78 & 219 \\
    & HUM & 0.44 & 0.56 / 0.56 / 0.56 & 0.72 & 0.82 & 333 \\
    \hline %&&&&&& \\
    \multirow{3}{*}{\tt !Rel} & S2T2 & 0.11 & 0.24 / 0.33 / 0.28 & 0.55 & 0.72 & 365 \\
     & GPT & 0.21 & 0.30 / 0.63 / 0.41 & 0.61 & 0.71 & 543 \\
     & HUM & 0.46 & 0.54 / 0.54 / 0.54 &0.73 & 0.85 & 261 \\
    \hline %&&&&&& \\
    \multirow{2}{*}{\tt !Par} & GPT & 0.13 & 0.27 / 0.14 / 0.19 & 0.56 & 0.89 & 79 \\
     & HUM & 0.45 & 0.49 / 0.49 / 0.49 & 0.72 & 0.91 & 151 \\
    \hline %&&&&&& \\
    \multirow{3}{*}{\tt !Sel} & DEC & 0.24 & 0.23 / 0.49 / 0.31 & 0.62 & 0.87 & 215 \\
    & GPT & 0.11 & 0.15 / 0.36 / 0.21 & 0.56 & 0.83 & 250 \\
    & HUM & 0.41 & 0.45 / 0.45 / 0.44 & 0.70 & 0.93 & 101 \\
    \hline %&&&&&& \\
    \multirow{3}{*}{\tt !Emp} & EPI & -0.03 & 0.12 / 0.15 / 0.13 & 0.48 & 0.72 & 291 \\
    & GPT & 0.09 & 0.21 / 0.36 / 0.27 & 0.55 & 0.72 & 396 \\
    & HUM & 0.44 & 0.52 / 0.52 / 0.52 & 0.72 & 0.86 & 231 \\
    \hline %&&&&&& \\
    \multirow{3}{*}{\tt Ign} & S2T2 & 0.11 & 0.18 / 0.40 / 0.25 & 0.55 & 0.75 & 365  \\
    & GPT & -0.02 & 0.16 / 0.63 / 0.25 & 0.49 & 0.60 & 696 \\
     & HUM & 0.57 & 0.62 / 0.62 / 0.62 & 0.79 & 0.92 & 170 \\
    \hline %&&&&&& \\
    \multirow{3}{*}{\tt Emp} & EPI & -0.14 & 0.40 / 0.86 / 0.54 & 0.43 & 0.45 & 1343 \\
    & GPT & -0.05 & 0.51 / 0.12 / 0.19 & 0.47 & 0.62 & 146 \\
     & HUM & 0.51 & 0.70 / 0.70 / 0.70 & 0.76 & 0.77 & 618 \\
    \end{tabular}
    }
    \caption{Error detection results on ABC-Eval. $\bm{\alpha}$: Krippendorf's alpha. \textbf{P$_+$ / R$_+$ / F1$_+$}: precision/recall/F1 on human-annotated positive labels. \textbf{F1}: macro F1. \textbf{Acc}: accuracy. \textbf{\#$_p$}: number of positive labels predicted by model. All human results (\textbf{HUM}) are calculated by comparing the 2 human annotators to each other. \textbf{Bold} indicates highest metric between automated classifiers for each behavior.}
    \label{tab:results}
\end{table}

==> latex/old/results_table_3.tex <==
\begin{table}[ht]
    \centering\small
    % \renewcommand{\arraystretch}{1.05}
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{r||l|r|l|l|l|l}
    & \bf Model & \multicolumn{1}{|c|}{\textbf{P$_+$ / R$_+$ / F1$_+$}}& \multicolumn{1}{|c|}{\textbf{P$_-$ / R$_-$ / F1$_-$}} & \bf Acc & \bf \#$\bm{_+}$ & \bf \#$\bm{_-}$ \\
    \hline \hline % &&&&&& \\
    \multirow{3}{*}{\tt !Fac} & FC & 0.12 / 0.22 / 0.16 & 0.93 / 0.87 / 0.90 & 0.82 & 223 & 1411 \\
    & GPT & 0.38 / 0.45 / 0.41 & 0.95 / 0.94 / 0.95 & 0.90 & 146 & 1488 \\
    & HUM & 0.68 / 0.68 / 0.68 & 0.97 / 0.97 / 0.97 & 0.95 & 122 & 1511 \\
    \hline %&&&&&& \\ 
    \multirow{2}{*}{\tt Red} & GPT & 0.31 / 0.35 / 0.33 & 0.94 / 0.93 / 0.94 & 0.89 & 148 & 1486 \\
    & HUM & 0.59 / 0.59 / 0.59 & 0.96 / 0.96 / 0.96 & 0.93 & 129 & 1504 \\
    \hline %&&&&&& \\
    \multirow{2}{*}{\tt !Com} & GPT & 0.44 / 0.29 / 0.35 & 0.83 / 0.91 / 0.87 & 0.78 & 219 & 1415 \\
    & HUM & 0.56 / 0.56 / 0.56 & 0.89 / 0.89 / 0.89 & 0.82 & 333 & 1301 \\
    \hline %&&&&&& \\
    \multirow{3}{*}{\tt !Rel} & S2T2 & 0.24 / 0.33 / 0.28 & 0.86 / 0.80 / 0.83 & 0.72 & 365 & 1269 \\
     & GPT & 0.30 / 0.63 / 0.41 & 0.91 / 0.72 / 0.81 & 0.71 & 543 & 1091 \\
     & HUM & 0.54 / 0.54 / 0.54 & 0.91 / 0.91 / 0.91 & 0.85 & 261 & 1372 \\
    \hline %&&&&&& \\
    \multirow{2}{*}{\tt !Par} & GPT & 0.27 / 0.14 / 0.19 & 0.92 / 0.96 / 0.94 & 0.89 & 79 & 1555 \\
     & HUM & 0.49 / 0.49 / 0.49 & 0.95 / 0.95 / 0.95 & 0.91 & 151 & 1482 \\
    \hline %&&&&&& \\
    \multirow{3}{*}{\tt !Sel} & DEC & 0.23 / 0.49 / 0.31 & 0.96 / 0.89 / 0.93 & 0.87 & 215 & 1419 \\
    & GPT & 0.15 / 0.36 / 0.21 & 0.95 / 0.86 / 0.90 & 0.83 & 250 & 1384 \\
    & HUM & 0.45 / 0.45 / 0.44 & 0.96 / 0.96 / 0.96 & 0.93 & 101 & 1532 \\
    \hline %&&&&&& \\
    \multirow{3}{*}{\tt !Emp} & EPI & 0.12 / 0.15 / 0.13 & 0.85 / 0.82 / 0.84 & 0.72 & 291 & 1343 \\
    & GPT & 0.21 / 0.36 / 0.27 & 0.88 / 0.78 / 0.83 & 0.72 & 396 & 1238 \\
    & HUM & 0.52 / 0.52 / 0.52 & 0.92 / 0.92 / 0.92 & 0.86 & 231 & 1403 \\
    \hline %&&&&&& \\
    \multirow{3}{*}{\tt Ign} & S2T2 & 0.18 / 0.40 / 0.25 & 0.92 / 0.80 / 0.85 & 0.75 & 365 & 1269  \\
    & GPT & 0.16 / 0.63 / 0.25 & 0.93 / 0.60 / 0.73 & 0.60 & 696 & 938 \\
     & HUM & 0.62 / 0.62 / 0.62 & 0.96 / 0.96 / 0.96 & 0.92 & 170 & 1463 \\
    \hline %&&&&&& \\
    \multirow{3}{*}{\tt Emp} & EPI & 0.40 / 0.86 / 0.54 & 0.70 / 0.20 / 0.31 & 0.45 & 1343 & 291 \\
    & GPT & 0.51 / 0.12 / 0.19 & 0.63 / 0.93 / 0.75 & 0.62 & 146 & 1488 \\
     & HUM & 0.70 / 0.70 / 0.70 & 0.82 / 0.82 / 0.82 & 0.77 & 618 & 1016 \\
    \end{tabular}
    }
    \caption{Error detection results on ABC-Eval. $\bm{\alpha}$: Krippendorf's alpha. \textbf{P$_+$ / R$_+$ / F1$_+$}: precision/recall/F1 on human-annotated positive labels. \textbf{F1}: macro F1. \textbf{Acc}: accuracy. \textbf{\#$_p$}: number of positive labels predicted by model. All human results (\textbf{HUM}) are calculated by comparing the 2 human annotators to each other. \textbf{Bold} indicates highest metric between automated classifiers for each behavior.}
    \label{tab:results}
\end{table}
